Pareto Manifold Learning: Tackling multiple tasks via ensembles of single-task models

In Multi-Task Learning (MTL), tasks may compete and limit the performance achieved on each other, rather than guiding the optimization to a solution, superior to all its single-task trained counterparts. Since there is often not a unique solution optimal for all tasks, practitioners have to balance tradeoffs between tasks' performance, and resort to optimality in the Pareto sense. Most MTL methodologies either completely neglect this aspect, and instead of aiming at learning a Pareto Front, produce one solution predefined by their optimization schemes, or produce diverse but discrete solutions. Recent approaches parameterize the Pareto Front via neural networks, leading to complex mappings from tradeoff to objective space. In this paper, we conjecture that the Pareto Front admits a linear parameterization in parameter space, which leads us to propose \textit{Pareto Manifold Learning}, an ensembling method in weight space. Our approach produces a continuous Pareto Front in a single training run, that allows to modulate the performance on each task during inference. Experiments on multi-task learning benchmarks, ranging from image classification to tabular datasets and scene understanding, show that \textit{Pareto Manifold Learning} outperforms state-of-the-art single-point algorithms, while learning a better Pareto parameterization than multi-point baselines.

==> sections/algo2.tex <==
\begin{algorithm}
\caption{\texttt{ParetoManifoldLearning} }
    % \Input{a}
    % \begin{algorithmic}[1]
\begin{algorithmic}[1]
    \REQUIRE matrix of model parameters  \( \bm{\Theta}=\begin{bmatrix}
        \nnparams{1} &\cdots&\nnparams{\numtasks}
    \end{bmatrix}^\top\), vector loss function \( \bm{L} \), train set \( \calD \), network \( f \), distribution parameters \( \pp\), window \( W\in\bbN \), regularization coefficient \( \lambda>0 \)

    \STATE Initialize each \( \nnparams{v} \) independently
    \STATE \( \calS_{\loss_1}\gets\varnothing \), \( \calS_{\loss_2}\gets\varnothing \)
    \FOR{batch \( (\xx, \yy) \subseteq \calD\) }
        \STATE \( \calV\gets\varnothing \)
        \FOR{ \( i \in \{1,2,\dots,W\}\) }
            \STATE sample  \( \aa_i \sim \textrm{Dir}(\pp) \) 
            \label{line:sampling}
            \STATE \( \calV\gets\calV\cup\aa_i \)
            \STATE \( \bmth_i\gets \aa_i ^\top  \bm{\Theta} \) 
            \label{line:construct convex hull} 
            \COMMENT{construct network in convex hull of ensemble members}
            \STATE \( \bm{L}(\aa_i) = \begin{bmatrix} \loss_1(\aa_i) &\cdots&\loss_\numtasks(\aa_i) \end{bmatrix}\gets \texttt{criterion}\left(f(\xx;\bmth_i), \yy \right) \) 
            \label{line:calculate loss} 
            \COMMENT{compute losses}
    %     }
        \ENDFOR
        %     % \( \calR_1\gets \sum_{t=1}^{T}\log\left( \frac{1}{{W \choose 2}} \sum_{i=1}^{W} \sum_{j>i}^{W} e^{\left[\kappa_t(\calL_t(\aa_i) -\calL_t(\aa_j))\right]_+ } \right)   \) \tcp*{multiforward regularization}
        \STATE construct multi-forward graphs \( \calG_t=(\calV,\calE_t) \)  \( \forall t\in[\numtasks] \) 
        \label{line:multiforward calc}
        \STATE \( \calR\gets \sum\limits_{t=1}^{T}\log\left( \frac{1}{|\calE_t|} \sum_{(\aa_i, \aa_j)\in\calE_t} e^{\left[\calL_t(\aa_i) -\calL_t(\aa_j)\right]_+ } \right)\label{line:reg multiforward}  \) 
        \COMMENT{multiforward regularization, \autoref{sec:algo extensions}}

        \STATE \( \loss_{\textrm{total}}\gets  \sum_{i=1}^{W} \aa_i ^\top \vectorloss(\aa_i) + \lambda \cdot  \calR\)\label{line:multiforward reg}
        \STATE Backpropagate \( \loss_{\textrm{total}} \) and Gradient \textit{descent} on \( \bm{\Theta} \)
    \ENDFOR
\end{algorithmic}
\end{algorithm}



% \begin{algorithm}[tb]
%     \caption{Bubble Sort}
%     \label{alg:example}
%  \begin{algorithmic}
%     \STATE {\bfseries Input:} data $x_i$, size $m$
%     \REPEAT
%     \STATE Initialize $noChange = true$.
%     \FOR{$i=1$ {\bfseries to} $m-1$}
%     \IF{$x_i > x_{i+1}$}
%     \STATE Swap $x_i$ and $x_{i+1}$
%     \STATE $noChange = false$
%     \ENDIF
%     \ENDFOR
%     \UNTIL{$noChange$ is $true$}
%  \end{algorithmic}
%  \end{algorithm}
 

==> sections/algo_copy.tex <==

\let\oldnl\nl
\newcommand{\nlnonumber}{\renewcommand{\nl}{\let\nl\oldnl}}
% \setlength{\algomargin}{11.5em}
    % \IncMargin{1.5em}
\begin{algorithm}[t]
    % \footnotesize
    \def\index{i}
    \DontPrintSemicolon
    \SetAlgoLined
    \SetAlCapHSkip{0pt} % Reset left skip of caption
    \setlength{\algomargin}{0em}
    % \setlength{\algomargin}{1.5em}
    
    % \Ind
    % \Input{
    %     vector loss function \( \bm{L} \), train set \( \calD \), network \( f \), matrix of model parameters  \( \bm{\Theta}=\begin{bmatrix}\nnparams{1},\cdots, \nnparams{\numtasks} \end{bmatrix}^\top\),   distribution parameters \( \pp\), window \( W\in\bbN \), regularization coefficient \( \lambda>0 \)
    % }
    \nlnonumber
    \textbf{Input: } vector loss function \( \bm{L} \), train set \( \calD \),  matrix of model parameters  \( \bm{\Theta}=\begin{bmatrix}\nnparams{1},\cdots, \nnparams{\numtasks} \end{bmatrix}^\top\),   distribution parameters \( \pp\), window \( W\in\bbN \), regularization coefficient \( \lambda>0 \), network \( f \)
    
    Initialize each \( \nnparams{v} \) independently
    % \Indp

    \For{batch \( (\xx, \yy) \subseteq \calD\) }{
        \( \calV\gets\varnothing \)

        \For{ \( i \in \{1,2,\dots,W\}\) }{
            sample  \( \aa_i \sim \textrm{Dir}(\pp) \) \label{line:sampling}

            \( \calV\gets\calV\cup\aa_i \)

            % \tcc*{construct network in convex hull of ensemble members}
            \( \bmth_i\gets \aa_i ^\top  \bm{\Theta} \) \label{line:construct convex hull} \tcp*{construct network in convex hull of ensemble members}

            \( \bm{L}(\aa_i) = \begin{bmatrix} \loss_1(\aa_i) &\cdots&\loss_\numtasks(\aa_i) \end{bmatrix}\gets \texttt{criterion}\left(f(\xx;\bmth_i), \yy \right) \) \label{line:calculate loss} \tcp*{compute losses}

        }
        construct multi-forward graphs \( \calG_t=(\calV,\calE_t), \forall t \) 
        \label{line:multiforward calc}

        \( \calR {\gets} \sum\limits_{t=1}^{T}\log\left( \frac{1}{|\calE_t|} \sum_{(\aa_i, \aa_j)\in\calE_t} e^{\left[\calL_t(\aa_i) -\calL_t(\aa_j)\right]_+ } \right)\label{line:reg multiforward}  \) \tcp*{multiforward regularization, \Autoref{sec:algo extensions}}
        % \( \calR\gets \sum\limits_{t=1}^{T}\log( \frac{1}{|\calE_t|} \sum_{(\aa_i, \aa_j)\in\calE_t} e^{\left[\calL_t(\aa_i) -\calL_t(\aa_j)\right]_+ } )\label{line:reg multiforward}  \) \tcp*{multiforward regularization, \Autoref{sec:algo extensions}}

        \( \loss_{\textrm{total}}\gets  \sum_{i=1}^{W} \aa_i ^\top \vectorloss(\aa_i) + \lambda \cdot  \calR\)\label{line:multiforward reg}

        Backpropagate \( \loss_{\textrm{total}} \) and 
        Gradient \textit{descent} on \( \bm{\Theta} \)
    }
    \caption{\small\texttt{ParetoManifoldLearning}}
    \label{algo:full}
\end{algorithm}



